Neural Refinement for Absolute Pose Regression with Feature Synthesis

Absolute Pose Regression (APR) methods use deep neural networks to directly regress camera poses from RGB images. However, the predominant APR architectures only rely on 2D operations during inference, resulting in limited accuracy of pose estimation due to the lack of 3D geometry constraints or priors. In this work, we propose a test-time refinement pipeline that leverages implicit geometric constraints using a robust feature field to enhance the ability of APR methods to use 3D information during inference. We also introduce a novel Neural Feature Synthesizer (NeFeS) model, which encodes 3D geometric features during training and directly renders dense novel view features at test time to refine APR methods. To enhance the robustness of our model, we introduce a feature fusion module and a progressive training strategy. Our proposed method achieves state-of-the-art single-image APR accuracy on indoor and outdoor datasets.

==> sec/06_ack.tex <==
\section{Acknowledgments}
Shuai Chen was supported by gift funding from Huawei UK. The authors also thank Wenjing Bian, Theo Costain for insightful discussions and proofreading.

==> table_tex/table7.tex <==
\begin{table}[t]
\centering
\resizebox{0.5\linewidth}{!}{

\begin{tabular}{lc}
            \toprule
            Method              & Church \\
            \midrule
            Combined & 0.35m/1.13\degree  \\
            Progressive & 0.32m/0.99\degree\\
            \bottomrule
        \end{tabular}
}
\caption{\textbf{Training Scheduling Ablation} Cambridge Church: Combined NeFeS Training vs. Progressive Training: 1. color, 2. feature, 3. fusion}
\label{table:7}
\end{table}

==> table_tex/table8.tex <==
% \begin{table}[t]
% \caption{\textbf{NFF vs. NeRF RGB+CNN} \cs{Improved results has not been updated yet}~}
% \label{table:8}
% \centering
% \resizebox{0.95\linewidth}{!}{
% \begin{tabular}{l|cc}
% \toprule
% Dataset   & RGB+CNN Features     & NFF Features  \\
% \midrule
% 7-Scenes   & 0.03/1.07      & \boldred{0.02}/\boldred{0.87}    \\
% Cambridge & \boldred{0.30}/0.77     & 0.35/\boldred{0.75}   \\
% \bottomrule
% \end{tabular}
% }
% \end{table}
